DyBit: Dynamic Bit-Precision Numbers for Efficient Quantized Neural Network Inference

To accelerate the inference of deep neural networks (DNNs), quantization with low-bitwidth numbers is actively researched. A prominent challenge is to quantize the DNN models into low-bitwidth numbers without significant accuracy degradation, especially at very low bitwidths (< 8 bits). This work targets an adaptive data representation with variable-length encoding called DyBit. DyBit can dynamically adjust the precision and range of separate bit-field to be adapted to the DNN weights/activations distribution. We also propose a hardware-aware quantization framework with a mixed-precision accelerator to trade-off the inference accuracy and speedup. Experimental results demonstrate that the inference accuracy via DyBit is 1.997% higher than the state-of-the-art at 4-bit quantization, and the proposed framework can achieve up to 8.1x speedup compared with the original model.

==> sec/01-intro-backup.tex <==
\section{Introduction}

Deep Learning (DL) approaches are widely applied for transformed representation learning in a variety of applications, including computer vision ~\cite{shapiro2001computer} and natural language processing ~\cite{floridi2020gpt}. Deep Neural Networks (DNNs) are now the main engine behind image processing and have been pushing the frontiers of many computer vision applications. For instance, the recent large Transformer-based Swim-B~\cite{liu2021swin} model has 88 million parameters and enormous computational complexity (47G FLOPs). Due to limited hardware resources and the need for real-time inference, efficiently deploying these DNN models has become a significant challenge, even in data centers. These challenges are more significant for edge/IoT devices with more constrained computation resources and energy consumption. 

%The size of DNN models increases by 120x each year, improving the AI hardware efficiency 2.5 times each year by IBM Research Center~\cite{joshi2020accurate}. However, the exact model size and capacity required for the task are still unknown, and a common strategy is to train overparameterized models and compress them into smaller representations. Model compression and acceleration methods such as tensor decomposition~\cite{sidiropoulos2017tensor}, pruning ~\cite{han2015deep,lin2021deformable}, and knowledge distillation~\cite{gou2021knowledge} target shrinking the network architectures while maintaining performance. 
% Deep Learning(DL) approaches are widely applied for transformed representation learning in a variety of applications, including computer vision ~\cite{shapiro2001computer} and natural language processing ~\cite{floridi2020gpt}. Convolutional Neural Networks (CNN) is now the main engine behind image processing and have been pushing the frontiers of many computer vision applications. Compared to their CNN counterparts, transformer-based models have larger receptive fields and are good at modeling long-range dependencies, which have been shown to achieve superior performance with large amounts of training data and model parameters. Specifically, the high number of keys involved in each query patch incurs high computational costs. For instance, the recent large Transformer-based Swim-B~\cite{liu2021swin} model has 88 million parameters and large computational complexity (47G FLOPs).  Due to limited resources (energy, memory footprint, and computation) and the need for real-time inference, the efficient deployment of these models has become a major challenge, even in data centers. Obviously, these challenges are greater for edge devices with more constrained computing and energy resources. The size of DNN models increases by 120x each year, improving the AI hardware efficiency 2.5 times each year by IBM Research Center~\cite{joshi2020accurate}. However, the exact model size and capacity required for the task are still unknown, and a common strategy is to train overparameterized models and compress them into smaller representations. 
% fig to illustrate the idea of the paper



\begin{figure}[htbp]
\centering
\includegraphics[scale=0.6]{figures/dac_figure1.pdf}
\caption{An illustration of different tensor distributions with Unified DyBit quantization model.}
\label{fig:dac_fig1}
\vspace{-1mm}
\end{figure}

% To achieve higher computational density and energy efficiency on these computing platforms, a number of quantization techniques with reduced precision and massive pruning methods have been proposed. 

Quantization is a practical approach to optimize DNN models in terms of low-latency and energy-efficient inference, since low-precision models can minimize data movement between memory hierarchies and reduces the area of computation units~\cite{johnson2018rethinking}. The quantized models usually achieve a typical speedup of 2-3x due to reduced precision for computations~\cite{nagel2021white}, compared with the original models based on floating-point numbers (FP). However, maintaining accuracy in very low precision ($\leq$ 8-bit) for DNN quantization becomes a challenge due to the linear distribution. Many previous works show that very low-precision integer quantization causes significant accuracy loss. To solve this problem, many low-bit-width data formats are proposed to achieve significant acceleration compared to original FP numbers while maintaining the inference accuracy. The critical approach is designing more adaptive formats specific for DNN quantization, in which the data representation can be dynamically adjusted for different layers/models, e.g., Posit~\cite{gustafson2017beating}, Adaptivfloat~\cite{adaptivfloat} and Flint~\cite{guo2022ant}.

Although low-precision adaptive data types make the DNN inference more efficient, another challenge is determining the bit-width of weights and activations for each layer based on a target hardware accelerator~\cite{wang2019haq}. Assuming there are $N$ bit-width selections for weights/activations, and the DNN model has $L$ layers, the total number of possible layer-wise solutions is $2 \times N^{L}$. In such a vast quantization space, automatically finding the optimal solution that meets the hardware constraints (e.g., hardware resource, memory size, minimal latency, etc.) becomes necessary, while the previous works with the adaptive data types did not discuss the fine-grained quantization space searching.

% Quantization is a practical approach to optimize DNN models in terms of low-latency and energy-efficient inference, since low-precision models can minimize data movement between memory hierarchies and reduces the area of computation circuit~\cite{johnson2018rethinking}. It is convenient for DNN inference since the network architecture remains unchanged and deploys quickly with various efficient methods. Quantized models usually achieve a typical speedup of 2-3x due to reduced precision for computations~\cite{nagel2021white}, compared with the original models based on floating-point numbers. Various computational arithmetic primitives represent values to save memory and computation. Some hardware accelerators are efficiently implemented on CPU/GPU ISAs, while others demand commercial hardware seek to improve floating-point itself with word size reduction, such as FP8/16~\cite{micikevicius2022fp8}, BF16~\cite{jouppi2017datacenter}, and TF32~\cite{nvidia2020a100} for \XX{efficient and accurate training}. One more efficient representation is the recent posit format for taper floating point by Gustafson~\cite{gustafson2017beating}. Ant's approach~\cite{guo2022ant} adopts the advantages of floating-point and integer formats. \XX{These fixed-length data formats cannot effectively quantize the DNN models according to the inter- and intra- layer distribution, which may degrade the model accuracy. Therefore, the variable-length decoding technique is a more efficient and accurate method to maintain original accuracy. Another challenge is that the variable-length quantization method requires special hardware support and the supported data format is also hardware-friendly.}

% Number systems and computer arithmetics are essential for designing efficient hardware and software architecture. In particular, real-valued computation constitutes a crucial component in almost all forms of today’s computing systems from mobile devices to servers. IEEE 754 is a prominent standard established in 1985 for representing real-valued numbers in a floating-point format. Despite all its benefits, this number system suffers from a number of weaknesses.

% fig to illustrate the idea of the paper
% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/dybit_version2.pdf}
% \caption{In this work, we propose the Dynamical Bit-level representation (DyBit) format. This format can dynamically adapt to the distribution of tensors, including dynamic precision and dynamic representation range.}
% \label{fig:idea_sum}
% \vspace{-5mm}
% \end{figure}

% Large size for small numbers. The IEEE 754 standard defines two specific formats for single- and double-precision value representation using 32 and 64 bits, respectively. Numerical computation within a limited range of values in these formats may be largely inefficient. For example, computing dot-products of values within [-1, 1] requires only a tiny fraction of all possible numbers represented in either format.
% Limited precision. IEEE 754 has predefined fixed-size partitions for an exponent and a fraction. This may lead to a rounding error when representing real numbers; therefore, some floating-point numbers are not precise.
% Exceptional bit representations. IEEE 754 reserves several bits to represent NaNs, denormals, positive/negative zero and infinity. In addition to wasting some of the possible bit patterns, considering all the reserved patterns for computation adds further complexity to the floating-point processors.
% Breaking algebraic rules. The floating-point formats may break algebraic rules during computation. For instance, a floating-point addition is not always associative. The expression (x+y)+z results in 1, where the floating-point values are x = 1e30, y = -1e30 and z = 1 is 1. Using the same values, x+(y+z) results in 0.
% All the above quantization works for network models that adopt the traditional data types such as int and float, but these types are inherently inefficient for DNN models. There are no optimal for most data distribution seen in neural network models in Fig.~\ref{fig:dac_fig1}. 

In this work, we \SG{propose} a run-length encoded data representation for low bit-width floating-point quantization to adapt the distribution of DNN parameters. This representation is based on a resilient and adaptive variable-length coding technique for encoding binary codes. Based on the adaptive strategy, we develop a hardware-aware framework that automatically quantizes the input DNN models for a given hardware accelerator. Thanks to the dynamically adaptive representation, our framework can quantize activations and weights to the lowest 4-bit and 2-bit, respectively, while maintaining higher accuracy compared with previous works. In addition, the proposed framework can be adapted to different application requirements. In scenarios with high real-time requirements, our framework can use latency as a constraint to obtain quantization with the smallest error, while in scenarios with high precision requirements, it can use quantization error as a constraint to obtain quantization with minimum latency. The key contributions of this work are:

% To overcome these challenges, our efficient quantization framework formulates a new encoding method to dynamically balance precision and representation range at the neural network level, adaptively adjust tensor distributions and match layer-wise DNN parameters. This is a resilient and adaptive variable-length coding technique for encoding binary codes. Compared with previous mixed-precision quantization works~\cite{sharma2018bit}, we have a more efficient hardware design and maintain good performance at low precision (i.e., 2,4-bit). Our experimental results prove that our accelerator can outperform BitFusion ~\cite{sharma2018bit}, with a 2$\times$ performance improvement. In this regard, we establish a link between a unified datatype and each tensor element with non-uniform distributions in Fig.~\ref{fig:dac_fig1}. The key contributions of this work are:

% To overcome these challenges, our unified quantization framework enacts a new datatype to dynamically balance precision and representation range at the neural network level, and it adaptively adjusts the tensor distribution and matches layer-wise DNN parameters. This is an elastic and adaptive bit-length coding technique for encoding integer and fractional bits. To reduce the quantization error, RMSE (Root Mean Square Error) is used to estimate the hyper-parameters in search spaces and the performance of DNNs. The generalized data format is supported by mixed-precision hardware accelerators.
\begin{itemize}
\item We propose \XX{a new dynamic bit-level data representation type}, \textit{DyBit}, which adopts dynamical precision and range bits at each tensor of DNNs to represent the distribution of parameters adaptively and develops a Bit-flexible variable length encoding algorithm for deep learning. 

\item We develop a run-time configurable mixed-precision accelerator specific for \textit{DyBit}. By fusing multiple multiply-accumulate operations (MAC) into one processing element, the accelerator significantly speeds up the DNN inference and reduces memory access.

\item We propose a hardware-aware quantization framework based on \textit{DyBit}. The proposed strategy searches for the optimal layer-wise quantization to get the maximum speed up under the constraints of quantization error. Evaluation results on several generic DNNs and transformer-based models show that our framework can achieve up to \XX{SP$\times$} speed up with an acceptable accuracy loss compared with the baseline quantization.

%in ImageNet Classification~\cite{deng2009imagenet}, and GLUE tasks~\cite{wang2018glue}.
% We conduct extensive experiments to verify our proposed quantization framework. It should be applicable to a large variety of tasks and models. 

\end{itemize} 

Recently, there has been a growing trend to accelerate deep neural network (DNN) inference. The pre-trained DNN models are generally based on high-precision floating-point (FP) numbers. Although the FP numbers give DNN models higher accuracy, it is challenging to conduct the fast inference, especially in embedded edge devices, since the accelerators have large computation overhead consumption and memory cost for the high-bitwidth FP data. To address this challenge, some recent works quantize the FP-based DNN models into linear fixed-point integers \cite{jacob2018quantization}. While significantly reducing the computation overhead and making the DNN inference faster, this approach suffers from significant accuracy degradation on very low bitwidths (<8bits) as different layers typically exhibit different resilience to quantization error. Some other works improve this defect by introducing mixed-precision quantization to adjust bitwidth in different parts of the neural network based on fixed-point numbers \cite{wang2019haq, li2021brecq, hao}. However, mixed-precision quantization can result in a vast search space for the optimal configuration \cite{wang2019haq}. Besides, it is also challenging to implement mixed-precision arithmetic on hardware without significant overhead, which may affect the acceleration effect \cite{wang2019haq}.
